Are LLMs Ready for Practical Adoption for Assertion Generation?

Assertions have been the de facto collateral for simulation-based and formal verification of hardware designs for over a decade. The quality of hardware verification, i.e., detection and diagnosis of corner-case design bugs, is critically dependent on the quality of the assertions. With the onset of generative AI such as Transformers and Large-Language Models (LLMs), there has been a renewed interest in developing novel, effective, and scalable techniques of generating functional and security assertions from design source code. While there have been recent works that use commercial-of-the-shelf (COTS) LLMs for assertion generation, there is no comprehensive study in quantifying the effectiveness of LLMs in generating syntactically and semantically correct assertions. In this paper, we first discuss AssertionBench from our prior work, a comprehensive set of designs and assertions to quantify the goodness of a broad spectrum of COTS LLMs for the task of assertion generations from hardware design source code. Our key insight was that COTS LLMs are not yet ready for prime-time adoption for assertion generation as they generate a considerable fraction of syntactically and semantically incorrect assertions. Motivated by the insight, we propose AssertionLLM, a first of its kind LLM model, specifically fine-tuned for assertion generation. Our initial experimental results show that AssertionLLM considerably improves the semantic and syntactic correctness of the generated assertions over COTS LLMs.

==> code/prompt_old.tex <==
\begin{comment}
You are an expert in SystemVerilog Assertions.
Your task is to generate the list of assertions to the given verilog design. An example is shown below. Generate only the list of assertions for the test program with no additional text.
Program 1: module arb2(clk, rst, req1, req2, gnt1, gnt2); input clk, rst; input req1, req2; output gnt1, gnt2; reg state; reg gnt1, gnt2; always @ (posedge clk or posedge rst) if (rst) state <= 0; else state <= gnt1; always @ (*) if (state) begin gnt1 = req1 & ~req2; gnt2 = req2; end else begin gnt1 = req1; gnt2 = req2 & ~req1; end endmodule
Assertions 1: (state == 1 & req2 == 1) |-> (gnt1 == 0);(req1 == 1 & state == 0) |-> (gnt1 == 1);(req1 == 0) |-> (gnt1 == 0);(req1 == 1 & req2 == 0) |-> (gnt1 == 1);(req1 == 1 & state == 0) |-> (gnt2 == 0);(req2 == 1 & state == 1) |-> (gnt2 == 1);(req2 == 0) |-> (gnt2 == 0);(req2 == 1 & req1 == 0) |-> (gnt2 == 1); (gnt2) |-> (req2); (gnt1) |-> (req1); 
Test Program: 
module fifo_mem #(parameter DEPTH=8, DATA_WIDTH=8, PTR_WIDTH=3) ( input wclk, w_en, rclk, r_en, input [PTR_WIDTH:0] b_wptr, b_rptr, input [DATA_WIDTH-1:0] data_in, input full, empty, output 
reg [DATA_WIDTH-1:0] data_out); reg [DATA_WIDTH-1:0] fifo[0:DEPTH-1]; always@(posedge wclk) begin if(w_en & !full) begin fifo[b_wptr[PTR_WIDTH-1:0]] <= data_in; end end always@(posedge rclk) begin  data_out <= fifo[b_rptr[PTR_WIDTH-1:0]]; end endmodule
Test Assertions:
\end{comment}

==> pic/comparative_results.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[]{}
%     \caption{Caption}
%     \label{fig:comparative_results}
% \end{figure}

==> table/Results_Vaishnavi_06052024_CSV_1.tex <==
fht\_1d\_x8 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.98 & 0.02 & 0.00 & 0.91 & 0.09 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.96 & 0.04 & 0.00 & 0.89 & 0.11 & 0.00 \\
fht\_8x8\_core & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.92 & 0.08 & 0.00 & 0.89 & 0.11 & 0.00 & 0.92 & 0.08 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
fht\_bfly & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.50 & 0.50 & 0.00 & 0.67 & 0.33 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 \\
fht\_bfly\_noFF & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.25 & 0.75 & 0.00 & 0.60 & 0.40 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
mtx\_trps\_8x8\_dpsram & 0.00 & 0.00 & 1.00 & 0.75 & 0.25 & 0 & 0.93 & 0.07 & 0.00 & 0.93 & 0.07 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.80 & 0.20 & 0.00 \\
signed\_mult\_const\_asic & 0.00 & 0.00 & 1.00 & 0.75 & 0.25 & 0 & 0.63 & 0.38 & 0.00 & 0.63 & 0.38 & 0.00 & 0.00 & 1.00 & 0.00 & 0.43 & 0.57 & 0.00 & 0.40 & 0.60 & 0.00 & 0.00 & 0.00 & 1.00 \\
signed\_mult\_const\_fpga & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.20 & 0.80 & 0.00 & 0.20 & 0.80 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
accumulatorMUX & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.86 & 0.14 & 0.00 & 0.86 & 0.14 & 0.00 & 0.67 & 0.33 & 0.00 & 0.67 & 0.33 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
bitNegator & 0.67 & 0.33 & 0.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 0.00 & 1.00 \\
ramBit & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.17 & 0.83 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.20 & 0.80 & 0.00 \\ \hline
byteNegator & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
ramByte & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.25 & 0.75 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
inputReg & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.01 & 0.99 & 0.00 & 0.00 & 0.00 & 1.00 \\
outputReg & 0.33 & 0.67 & 0.00 & 1.00 & 0.00 & 0 & 0.57 & 0.43 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
ppReg1 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
tcLoad & 0.75 & 0.25 & 0.00 & 0.50 & 0.50 & 0 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.63 & 0.38 & 0.00 & 1.00 & 0.00 & 0.00 & 0.16 & 0.84 & 0.00 \\
tcReset & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0 & 0.75 & 0.25 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.14 & 0.86 & 0.00 & 0.00 & 0.00 & 1.00 \\
uartRec & 0.00 & 1.00 & 0.00 & 0.18 & 0.82 & 0 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.36 & 0.64 & 0.00 & 0.00 & 0.00 & 1.00 & 0.14 & 0.86 & 0.00 & 0.92 & 0.08 & 0.00 \\
uartTrans & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.86 & 0.14 & 0.00 & 1.00 & 0.00 & 0.00 & 0.35 & 0.65 & 0.00 & 0.00 & 0.00 & 1.00 & 0.68 & 0.32 & 0.00 & 0.53 & 0.47 & 0.00 \\
host\_interface\_aes & 0.00 & 0.00 & 1.00 & 0.21 & 0.79 & 0 & 0.64 & 0.36 & 0.00 & 0.60 & 0.40 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.31 & 0.69 & 0.00 & 0.13 & 0.88 & 0.00 \\ \hline
key\_expander & 0.38 & 0.63 & 0.00 & 0.29 & 0.71 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.28 & 0.72 & 0.00 & 0.00 & 0.00 & 1.00 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 \\
clc\_fsm & 1.00 & 0.00 & 0.00 & 0.91 & 0.09 & 0 & 0.93 & 0.07 & 0.00 & 0.93 & 0.07 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
clc\_len\_gen & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
clc\_read\_lels & 0.25 & 0.75 & 0.00 & 0.64 & 0.36 & 0 & 0.00 & 0.00 & 1.00 & 0.31 & 0.69 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.94 & 0.06 & 0.00 & 1.00 & 0.00 & 0.00 \\
clc\_read\_total\_coeffs & 0.74 & 0.26 & 0.00 & 0.36 & 0.64 & 0 & 0.64 & 0.36 & 0.00 & 0.74 & 0.26 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
clc\_read\_total\_zeros & 0.14 & 0.86 & 0.00 & 0.03 & 0.97 & 0 & 0.39 & 0.61 & 0.00 & 0.39 & 0.61 & 0.00 & 0.35 & 0.65 & 0.00 & 0.14 & 0.86 & 0.00 & 0.04 & 0.96 & 0.00 & 0.00 & 1.00 & 0.00 \\
ca\_prng & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.89 & 0.11 & 0.00 & 0.41 & 0.59 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0.00 & 0.19 & 0.81 & 0.00 \\
mux4to1 & 0.33 & 0.67 & 0.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.29 & 0.71 & 0.00 & 0.20 & 0.80 & 0.00 \\
PSGBusArb & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 0.00 & 1.00 & 0.00 & 0.11 & 0.89 & 0.00 & 0.50 & 0.50 & 0.00 & 0.94 & 0.06 & 0.00 & 0.56 & 0.44 & 0.00 & 1.00 & 0.00 & 0.00 \\
PSGChannelSummer & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\ \hline
PSGFilter & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0 & 0.09 & 0.91 & 0.00 & 0.09 & 0.91 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
PSGMasterVolumeControl & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.17 & 0.83 & 0.00 & 0.08 & 0.92 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
PSGOutputSummer & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 \\
PSGShaper & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
bit\_rersal & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.13 & 0.88 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0.00 & 0.25 & 0.75 & 0.00 \\
crc\_comb & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.94 & 0.06 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.20 & 0.80 & 0.00 \\
crc\_control\_unit & 0.59 & 0.41 & 0.00 & 0.00 & 1.00 & 0 & 1.00 & 0.00 & 0.00 & 0.93 & 0.07 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.84 & 0.16 & 0.00 & 0.93 & 0.07 & 0.00 \\
host\_interface & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0 & 0.75 & 0.25 & 0.00 & 0.79 & 0.21 & 0.00 & 0.00 & 1.00 & 0.00 & 0.63 & 0.38 & 0.00 & 0.00 & 1.00 & 0.00 & 0.64 & 0.36 & 0.00 \\
fpu\_exceptions & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.68 & 0.32 & 0.00 & 0.00 & 0.00 & 1.00 \\
fpu\_sub & 0.00 & 1.00 & 0.00 & 0.17 & 0.83 & 0 & 0.00 & 1.00 & 0.00 & 0.03 & 0.97 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\ \hline
qadd & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 0.80 & 0.20 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.75 & 0.25 & 0.00 & 0.75 & 0.25 & 0.00 & 0.00 & 0.00 & 1.00 \\
qmult & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0 & 0.89 & 0.11 & 0.00 & 0.78 & 0.22 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.95 & 0.05 & 0.00 & 0.29 & 0.71 & 0.00 \\
qtwosComp & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.10 & 0.90 & 0.00 & 0.17 & 0.83 & 0.00 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
dff\_3\_pipe & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0 & 0.50 & 0.50 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0.00 & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0.00 \\
node & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0.00 \\
dpll & 0.36 & 0.64 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.10 & 0.90 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 & 0.24 & 0.76 & 0.00 \\
freqdider & 0.00 & 1.00 & 0.00 & 0.17 & 0.83 & 0 & 0.00 & 1.00 & 0.00 & 0.20 & 0.80 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
variableresetrandomwalkfilter & 0.00 & 0.00 & 1.00 & 0.73 & 0.27 & 0 & 0.37 & 0.63 & 0.00 & 0.41 & 0.59 & 0.00 & 0.39 & 0.61 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.83 & 0.17 & 0.00 \\
clean\_rst & 0.50 & 0.50 & 0.00 & 0.67 & 0.33 & 0 & 0.33 & 0.67 & 0.00 & 0.40 & 0.60 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.60 & 0.40 & 0.00 & 0.29 & 0.71 & 0.00 \\
decoder\_8b10b & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.03 & 0.97 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.33 & 0.67 & 0.00 & 0.19 & 0.81 & 0.00 \\ \hline
encoder\_8b10b & 0.00 & 0.00 & 1.00 & 0.19 & 0.81 & 0 & 0.25 & 0.75 & 0.00 & 0.11 & 0.89 & 0.00 & 0.42 & 0.58 & 0.00 & 0.79 & 0.21 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
ge\_1000baseX\_mdio & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.71 & 0.29 & 0.00 & 0.00 & 0.00 & 1.00 \\
ge\_1000baseX\_rx & 0.19 & 0.81 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.64 & 0.36 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
ge\_1000baseX\_sync & 0.26 & 0.74 & 0.00 & 0.18 & 0.82 & 0 & 0.38 & 0.63 & 0.00 & 0.27 & 0.73 & 0.00 & 0.27 & 0.73 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.12 & 0.88 & 0.00 \\
eth\_cop & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
eth\_crc & 0.00 & 1.00 & 0.00 & 0.75 & 0.25 & 0 & 0.26 & 0.74 & 0.00 & 0.27 & 0.73 & 0.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 1.00 & 0.00 & 0.14 & 0.86 & 0.00 \\
eth\_l3\_checksum & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 \\
eth\_random & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.67 & 0.33 & 0.00 & 0.93 & 0.07 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.67 & 0.33 & 0.00 & 0.43 & 0.57 & 0.00 \\
eth\_receecontrol & 0.55 & 0.45 & 0.00 & 0.58 & 0.42 & 0 & 0.52 & 0.48 & 0.00 & 0.28 & 0.72 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.45 & 0.55 & 0.00 \\
eth\_rxaddrcheck & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 1.00 & 0.00 & 0.24 & 0.76 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\ \hline
eth\_clockgen & 0.00 & 0.00 & 1.00 & 0.67 & 0.33 & 0 & 0.60 & 0.40 & 0.00 & 0.67 & 0.33 & 0.00 & 0.00 & 1.00 & 0.00 & 0.67 & 0.33 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
eth\_miim & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.54 & 0.46 & 0.00 & 0.52 & 0.48 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
eth\_outputcontrol & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.43 & 0.57 & 0.00 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 & 0.14 & 0.86 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
eth\_shiftreg & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.33 & 0.67 & 0.00 & 0.20 & 0.80 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
flow\_ctrl & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0 & 0.53 & 0.47 & 0.00 & 0.10 & 0.90 & 0.00 & 0.19 & 0.81 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
MAC\_rx\_ctrl & 0.00 & 0.00 & 1.00 & 0.25 & 0.75 & 0 & 0.78 & 0.23 & 0.00 & 0.79 & 0.21 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.30 & 0.70 & 0.00 \\
Phy\_sim & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.38 & 0.63 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
Ramdon\_gen & 0.00 & 0.00 & 1.00 & 0.25 & 0.75 & 0 & 0.70 & 0.30 & 0.00 & 0.70 & 0.30 & 0.00 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 & 0.73 & 0.27 & 0.00 & 0.08 & 0.92 & 0.00 \\
reg\_int\_sim & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.71 & 0.29 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
RMON\_addr\_gen & 0.00 & 0.00 & 1.00 & 0.23 & 0.77 & 0 & 0.00 & 0.00 & 1.00 & 0.40 & 0.60 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.44 & 0.56 & 0.00 & 0.00 & 1.00 & 0.00 \\ \hline
RMON\_ctrl & 0.00 & 0.00 & 1.00 & 0.61 & 0.39 & 0 & 0.76 & 0.24 & 0.00 & 0.78 & 0.23 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.33 & 0.67 & 0.00 & 0.52 & 0.48 & 0.00 \\
ack\_counter & 0.00 & 0.00 & 1.00 & 0.56 & 0.44 & 0 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 & 0.17 & 0.83 & 0.00 & 0.14 & 0.86 & 0.00 & 0.10 & 0.90 & 0.00 & 0.13 & 0.87 & 0.00 \\
counter & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0 & 0.50 & 0.50 & 0.00 & 0.56 & 0.44 & 0.00 & 0.33 & 0.67 & 0.00 & 0.33 & 0.67 & 0.00 & 0.43 & 0.57 & 0.00 & 0.00 & 0.00 & 1.00 \\
rxClkgen & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 \\
rxLinkFaultState & 0.00 & 0.00 & 1.00 & 0.29 & 0.71 & 0 & 0.20 & 0.80 & 0.00 & 0.20 & 0.80 & 0.00 & 0.26 & 0.74 & 0.00 & 0.33 & 0.67 & 0.00 & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0.00 \\
rxNumCounter & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0 & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.97 & 0.03 & 0.00 \\
rxStateMachine & 0.00 & 0.00 & 1.00 & 0.67 & 0.33 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.71 & 0.29 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
rxStatModule & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 0.06 & 0.94 & 0.00 & 0.06 & 0.94 & 0.00 & 0.06 & 0.94 & 0.00 & 0.06 & 0.94 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 \\
apb & 0.17 & 0.83 & 0.00 & 0.73 & 0.27 & 0 & 0.73 & 0.27 & 0.00 & 0.73 & 0.27 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.40 & 0.60 & 0.00 \\
can\_btl & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.15 & 0.85 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\ \hline
can\_crc & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.43 & 0.57 & 0.00 \\
can\_fifo & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.29 & 0.71 & 0.00 & 0.29 & 0.71 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.03 & 0.97 & 0.00 \\
can\_ibo & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
can\_register\_asyn & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
can\_register\_asyn\_syn & 0.50 & 0.50 & 0.00 & 0.25 & 0.75 & 0 & 0.40 & 0.60 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 & 0.33 & 0.67 & 0.00 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 \\
can\_register & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
can\_register\_syn & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
can\_acf & 0.00 & 1.00 & 0.00 & 0.29 & 0.71 & 0 & 0.00 & 1.00 & 0.00 & 0.14 & 0.86 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.04 & 0.96 & 0.00 \\
eth\_fifo & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.19 & 0.81 & 0.00 & 0.17 & 0.83 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
Phy\_int & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.29 & 0.71 & 0.00 & 0.31 & 0.69 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.33 & 0.67 & 0.00 & 0.05 & 0.95 & 0.00 \\ \hline
% fpu\_add & 0.17 & 0.83 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.08 & 0.92 & 0.00 & 0.00 & 1.00 & 0.00 & 0.15 & 0.85 & 0.00 \\
% control\_unit & 0.00 & 0.00 & 1.00 & 0.93 & 0.07 & 0 & 0.95 & 0.05 & 0.00 & 0.95 & 0.05 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 0.99 & 0.01 & 0.00 & 1.00 & 0.00 & 0.00 \\
% phasecomparator & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% wptr\_handler & 0.71 & 0.29 & 0.00 & 1.00 & 0.00 & 0 & 0.00 & 0.00 & 1.00 & 0.90 & 0.10 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.00 & 0.00 & 1.00 & 0.83 & 0.17 & 0.00 \\
% rptr\_handler & 1.00 & 0.00 & 0.00 & 0.86 & 0.14 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.89 & 0.11 & 0.00 & 0.86 & 0.14 & 0.00 \\
% synchronizer & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.60 & 0.40 & 0.00 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.13 & 0.88 & 0.00 & 0.11 & 0.89 & 0.00 \\
% fifo\_mem & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% MAC\_tx\_Ctrl & 0.18 & 0.82 & 0.00 & 0.00 & 1.00 & 0 & 0.67 & 0.33 & 0.00 & 0.74 & 0.26 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.58 & 0.42 & 0.00 & 0.55 & 0.45 & 0.00 \\


==> table/Results_Vaishnavi_06052024_CSV_2.tex <==
% fht\_1d\_x8 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.98 & 0.02 & 0.00 & 0.91 & 0.09 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.96 & 0.04 & 0.00 & 0.89 & 0.11 & 0.00 \\
% fht\_8x8\_core & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.92 & 0.08 & 0.00 & 0.89 & 0.11 & 0.00 & 0.92 & 0.08 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% fht\_bfly & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.50 & 0.50 & 0.00 & 0.67 & 0.33 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 \\
% fht\_bfly\_noFF & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.25 & 0.75 & 0.00 & 0.60 & 0.40 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
% mtx\_trps\_8x8\_dpsram & 0.00 & 0.00 & 1.00 & 0.75 & 0.25 & 0 & 0.93 & 0.07 & 0.00 & 0.93 & 0.07 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.80 & 0.20 & 0.00 \\
% signed\_mult\_const\_asic & 0.00 & 0.00 & 1.00 & 0.75 & 0.25 & 0 & 0.63 & 0.38 & 0.00 & 0.63 & 0.38 & 0.00 & 0.00 & 1.00 & 0.00 & 0.43 & 0.57 & 0.00 & 0.40 & 0.60 & 0.00 & 0.00 & 0.00 & 1.00 \\
% signed\_mult\_const\_fpga & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.20 & 0.80 & 0.00 & 0.20 & 0.80 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% accumulatorMUX & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.86 & 0.14 & 0.00 & 0.86 & 0.14 & 0.00 & 0.67 & 0.33 & 0.00 & 0.67 & 0.33 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% bitNegator & 0.67 & 0.33 & 0.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 0.00 & 1.00 \\
% ramBit & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.17 & 0.83 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.20 & 0.80 & 0.00 \\ \hline
% byteNegator & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% ramByte & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.25 & 0.75 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% inputReg & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.01 & 0.99 & 0.00 & 0.00 & 0.00 & 1.00 \\
% outputReg & 0.33 & 0.67 & 0.00 & 1.00 & 0.00 & 0 & 0.57 & 0.43 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% ppReg1 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% tcLoad & 0.75 & 0.25 & 0.00 & 0.50 & 0.50 & 0 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.63 & 0.38 & 0.00 & 1.00 & 0.00 & 0.00 & 0.16 & 0.84 & 0.00 \\
% tcReset & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0 & 0.75 & 0.25 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.14 & 0.86 & 0.00 & 0.00 & 0.00 & 1.00 \\
% uartRec & 0.00 & 1.00 & 0.00 & 0.18 & 0.82 & 0 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.36 & 0.64 & 0.00 & 0.00 & 0.00 & 1.00 & 0.14 & 0.86 & 0.00 & 0.92 & 0.08 & 0.00 \\
% uartTrans & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.86 & 0.14 & 0.00 & 1.00 & 0.00 & 0.00 & 0.35 & 0.65 & 0.00 & 0.00 & 0.00 & 1.00 & 0.68 & 0.32 & 0.00 & 0.53 & 0.47 & 0.00 \\
% host\_interface\_aes & 0.00 & 0.00 & 1.00 & 0.21 & 0.79 & 0 & 0.64 & 0.36 & 0.00 & 0.60 & 0.40 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.31 & 0.69 & 0.00 & 0.13 & 0.88 & 0.00 \\ \hline
% key\_expander & 0.38 & 0.63 & 0.00 & 0.29 & 0.71 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.28 & 0.72 & 0.00 & 0.00 & 0.00 & 1.00 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 \\
% clc\_fsm & 1.00 & 0.00 & 0.00 & 0.91 & 0.09 & 0 & 0.93 & 0.07 & 0.00 & 0.93 & 0.07 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
% clc\_len\_gen & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
% clc\_read\_lels & 0.25 & 0.75 & 0.00 & 0.64 & 0.36 & 0 & 0.00 & 0.00 & 1.00 & 0.31 & 0.69 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.94 & 0.06 & 0.00 & 1.00 & 0.00 & 0.00 \\
% clc\_read\_total\_coeffs & 0.74 & 0.26 & 0.00 & 0.36 & 0.64 & 0 & 0.64 & 0.36 & 0.00 & 0.74 & 0.26 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
% clc\_read\_total\_zeros & 0.14 & 0.86 & 0.00 & 0.03 & 0.97 & 0 & 0.39 & 0.61 & 0.00 & 0.39 & 0.61 & 0.00 & 0.35 & 0.65 & 0.00 & 0.14 & 0.86 & 0.00 & 0.04 & 0.96 & 0.00 & 0.00 & 1.00 & 0.00 \\
% ca\_prng & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.89 & 0.11 & 0.00 & 0.41 & 0.59 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0.00 & 0.19 & 0.81 & 0.00 \\
% mux4to1 & 0.33 & 0.67 & 0.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.29 & 0.71 & 0.00 & 0.20 & 0.80 & 0.00 \\
% PSGBusArb & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 0.00 & 1.00 & 0.00 & 0.11 & 0.89 & 0.00 & 0.50 & 0.50 & 0.00 & 0.94 & 0.06 & 0.00 & 0.56 & 0.44 & 0.00 & 1.00 & 0.00 & 0.00 \\
% PSGChannelSummer & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\ \hline
% PSGFilter & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0 & 0.09 & 0.91 & 0.00 & 0.09 & 0.91 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% PSGMasterVolumeControl & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.17 & 0.83 & 0.00 & 0.08 & 0.92 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% PSGOutputSummer & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 \\
% PSGShaper & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% bit\_rersal & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.13 & 0.88 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0.00 & 0.25 & 0.75 & 0.00 \\
% crc\_comb & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.94 & 0.06 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.20 & 0.80 & 0.00 \\
% crc\_control\_unit & 0.59 & 0.41 & 0.00 & 0.00 & 1.00 & 0 & 1.00 & 0.00 & 0.00 & 0.93 & 0.07 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.84 & 0.16 & 0.00 & 0.93 & 0.07 & 0.00 \\
% host\_interface & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0 & 0.75 & 0.25 & 0.00 & 0.79 & 0.21 & 0.00 & 0.00 & 1.00 & 0.00 & 0.63 & 0.38 & 0.00 & 0.00 & 1.00 & 0.00 & 0.64 & 0.36 & 0.00 \\
% fpu\_exceptions & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.68 & 0.32 & 0.00 & 0.00 & 0.00 & 1.00 \\
% fpu\_sub & 0.00 & 1.00 & 0.00 & 0.17 & 0.83 & 0 & 0.00 & 1.00 & 0.00 & 0.03 & 0.97 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\ \hline
% qadd & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 0.80 & 0.20 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.75 & 0.25 & 0.00 & 0.75 & 0.25 & 0.00 & 0.00 & 0.00 & 1.00 \\
% qmult & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0 & 0.89 & 0.11 & 0.00 & 0.78 & 0.22 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.95 & 0.05 & 0.00 & 0.29 & 0.71 & 0.00 \\
% qtwosComp & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.10 & 0.90 & 0.00 & 0.17 & 0.83 & 0.00 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% dff\_3\_pipe & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0 & 0.50 & 0.50 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0.00 & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0.00 \\
% node & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.50 & 0.50 & 0.00 \\
% dpll & 0.36 & 0.64 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.10 & 0.90 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 & 0.24 & 0.76 & 0.00 \\
% freqdider & 0.00 & 1.00 & 0.00 & 0.17 & 0.83 & 0 & 0.00 & 1.00 & 0.00 & 0.20 & 0.80 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% variableresetrandomwalkfilter & 0.00 & 0.00 & 1.00 & 0.73 & 0.27 & 0 & 0.37 & 0.63 & 0.00 & 0.41 & 0.59 & 0.00 & 0.39 & 0.61 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.83 & 0.17 & 0.00 \\
% clean\_rst & 0.50 & 0.50 & 0.00 & 0.67 & 0.33 & 0 & 0.33 & 0.67 & 0.00 & 0.40 & 0.60 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.60 & 0.40 & 0.00 & 0.29 & 0.71 & 0.00 \\
% decoder\_8b10b & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.03 & 0.97 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.33 & 0.67 & 0.00 & 0.19 & 0.81 & 0.00 \\ \hline
% encoder\_8b10b & 0.00 & 0.00 & 1.00 & 0.19 & 0.81 & 0 & 0.25 & 0.75 & 0.00 & 0.11 & 0.89 & 0.00 & 0.42 & 0.58 & 0.00 & 0.79 & 0.21 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% ge\_1000baseX\_mdio & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.71 & 0.29 & 0.00 & 0.00 & 0.00 & 1.00 \\
% ge\_1000baseX\_rx & 0.19 & 0.81 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.64 & 0.36 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
% ge\_1000baseX\_sync & 0.26 & 0.74 & 0.00 & 0.18 & 0.82 & 0 & 0.38 & 0.63 & 0.00 & 0.27 & 0.73 & 0.00 & 0.27 & 0.73 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.12 & 0.88 & 0.00 \\
% eth\_cop & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% eth\_crc & 0.00 & 1.00 & 0.00 & 0.75 & 0.25 & 0 & 0.26 & 0.74 & 0.00 & 0.27 & 0.73 & 0.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 1.00 & 0.00 & 0.14 & 0.86 & 0.00 \\
% eth\_l3\_checksum & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 \\
% eth\_random & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.67 & 0.33 & 0.00 & 0.93 & 0.07 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.67 & 0.33 & 0.00 & 0.43 & 0.57 & 0.00 \\
% eth\_receecontrol & 0.55 & 0.45 & 0.00 & 0.58 & 0.42 & 0 & 0.52 & 0.48 & 0.00 & 0.28 & 0.72 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.45 & 0.55 & 0.00 \\
% eth\_rxaddrcheck & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.00 & 1.00 & 0.00 & 0.24 & 0.76 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\ \hline
% eth\_clockgen & 0.00 & 0.00 & 1.00 & 0.67 & 0.33 & 0 & 0.60 & 0.40 & 0.00 & 0.67 & 0.33 & 0.00 & 0.00 & 1.00 & 0.00 & 0.67 & 0.33 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% eth\_miim & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.54 & 0.46 & 0.00 & 0.52 & 0.48 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% eth\_outputcontrol & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.43 & 0.57 & 0.00 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 & 0.14 & 0.86 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
% eth\_shiftreg & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.33 & 0.67 & 0.00 & 0.20 & 0.80 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% flow\_ctrl & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0 & 0.53 & 0.47 & 0.00 & 0.10 & 0.90 & 0.00 & 0.19 & 0.81 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% MAC\_rx\_ctrl & 0.00 & 0.00 & 1.00 & 0.25 & 0.75 & 0 & 0.78 & 0.23 & 0.00 & 0.79 & 0.21 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.30 & 0.70 & 0.00 \\
% Phy\_sim & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.38 & 0.63 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 \\
% Ramdon\_gen & 0.00 & 0.00 & 1.00 & 0.25 & 0.75 & 0 & 0.70 & 0.30 & 0.00 & 0.70 & 0.30 & 0.00 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 & 0.73 & 0.27 & 0.00 & 0.08 & 0.92 & 0.00 \\
% reg\_int\_sim & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 0.71 & 0.29 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
% RMON\_addr\_gen & 0.00 & 0.00 & 1.00 & 0.23 & 0.77 & 0 & 0.00 & 0.00 & 1.00 & 0.40 & 0.60 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.44 & 0.56 & 0.00 & 0.00 & 1.00 & 0.00 \\ \hline
% RMON\_ctrl & 0.00 & 0.00 & 1.00 & 0.61 & 0.39 & 0 & 0.76 & 0.24 & 0.00 & 0.78 & 0.23 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.33 & 0.67 & 0.00 & 0.52 & 0.48 & 0.00 \\
% ack\_counter & 0.00 & 0.00 & 1.00 & 0.56 & 0.44 & 0 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 & 0.17 & 0.83 & 0.00 & 0.14 & 0.86 & 0.00 & 0.10 & 0.90 & 0.00 & 0.13 & 0.87 & 0.00 \\
% counter & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0 & 0.50 & 0.50 & 0.00 & 0.56 & 0.44 & 0.00 & 0.33 & 0.67 & 0.00 & 0.33 & 0.67 & 0.00 & 0.43 & 0.57 & 0.00 & 0.00 & 0.00 & 1.00 \\
% rxClkgen & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 \\
% rxLinkFaultState & 0.00 & 0.00 & 1.00 & 0.29 & 0.71 & 0 & 0.20 & 0.80 & 0.00 & 0.20 & 0.80 & 0.00 & 0.26 & 0.74 & 0.00 & 0.33 & 0.67 & 0.00 & 0.00 & 0.00 & 1.00 & 0.50 & 0.50 & 0.00 \\
% rxNumCounter & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0 & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.97 & 0.03 & 0.00 \\
% rxStateMachine & 0.00 & 0.00 & 1.00 & 0.67 & 0.33 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.71 & 0.29 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% rxStatModule & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0 & 0.06 & 0.94 & 0.00 & 0.06 & 0.94 & 0.00 & 0.06 & 0.94 & 0.00 & 0.06 & 0.94 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 \\
% apb & 0.17 & 0.83 & 0.00 & 0.73 & 0.27 & 0 & 0.73 & 0.27 & 0.00 & 0.73 & 0.27 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.40 & 0.60 & 0.00 \\
% can\_btl & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.15 & 0.85 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\ \hline
% can\_crc & 0.00 & 0.00 & 1.00 & 0.20 & 0.80 & 0 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.25 & 0.75 & 0.00 & 0.43 & 0.57 & 0.00 \\
% can\_fifo & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1 & 0.29 & 0.71 & 0.00 & 0.29 & 0.71 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.03 & 0.97 & 0.00 \\
% can\_ibo & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 \\
% can\_register\_asyn & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.50 & 0.50 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% can\_register\_asyn\_syn & 0.50 & 0.50 & 0.00 & 0.25 & 0.75 & 0 & 0.40 & 0.60 & 0.00 & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0.00 & 0.33 & 0.67 & 0.00 & 0.50 & 0.50 & 0.00 & 0.50 & 0.50 & 0.00 \\
% can\_register & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% can\_register\_syn & 0.25 & 0.75 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% can\_acf & 0.00 & 1.00 & 0.00 & 0.29 & 0.71 & 0 & 0.00 & 1.00 & 0.00 & 0.14 & 0.86 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.04 & 0.96 & 0.00 \\
% eth\_fifo & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.19 & 0.81 & 0.00 & 0.17 & 0.83 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
% Phy\_int & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.29 & 0.71 & 0.00 & 0.31 & 0.69 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.33 & 0.67 & 0.00 & 0.05 & 0.95 & 0.00 \\ \hline
fpu\_add & 0.17 & 0.83 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.08 & 0.92 & 0.00 & 0.00 & 1.00 & 0.00 & 0.15 & 0.85 & 0.00 \\
control\_unit & 0.00 & 0.00 & 1.00 & 0.93 & 0.07 & 0 & 0.95 & 0.05 & 0.00 & 0.95 & 0.05 & 0.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 0.99 & 0.01 & 0.00 & 1.00 & 0.00 & 0.00 \\
phasecomparator & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 \\
wptr\_handler & 0.71 & 0.29 & 0.00 & 1.00 & 0.00 & 0 & 0.00 & 0.00 & 1.00 & 0.90 & 0.10 & 0.00 & 1.00 & 0.00 & 0.00 & 0.75 & 0.25 & 0.00 & 0.00 & 0.00 & 1.00 & 0.83 & 0.17 & 0.00 \\
rptr\_handler & 1.00 & 0.00 & 0.00 & 0.86 & 0.14 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.89 & 0.11 & 0.00 & 0.86 & 0.14 & 0.00 \\
synchronizer & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.60 & 0.40 & 0.00 & 0.33 & 0.67 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.13 & 0.88 & 0.00 & 0.11 & 0.89 & 0.00 \\
fifo\_mem & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
MAC\_tx\_Ctrl & 0.18 & 0.82 & 0.00 & 0.00 & 1.00 & 0 & 0.67 & 0.33 & 0.00 & 0.74 & 0.26 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.00 & 0.58 & 0.42 & 0.00 & 0.55 & 0.45 & 0.00 \\ \hline


==> table/post_syntactic_correction.tex <==
\begin{table}
    \centering
    \caption{{\bf Comparative results for four different commercial and open-source LLMs using 1-shot and 5-shot learning for the assertion generation task}. {\bf P}: Fraction of proven assertions. {\bf C}: Fraction of failed assertions with a counter-example. {\bf E}: Fraction of assertions which have syntax errors.}
    \label{tab:result_after_syn_correction}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
         \hline
         \multirow{2}{*}{\bf Designs} & \multicolumn{6}{|c|}{\bf ChatGPT 3.5} & \multicolumn{6}{|c|}{\bf ChatGPT 4.0} & \multicolumn{6}{|c|}{\bf CodeLLaMa2} & \multicolumn{6}{|c|}{\bf LLaMa3-70B} \\
         \cline{2-25}
         \multirow{2}{*}{} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} \\
         \cline{2-25}
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E}
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E} \\
         \hline
         \input{table/Results_Vaishnavi_06052024_CSV_1}
    \end{tabular}
    }
\end{table}

\begin{table}
    \centering
    \caption{{\bf Comparative results for four different commercial and open-source LLMs using 1-shot and 5-shot learning for the assertion generation task}. {\bf P}: Fraction of proven assertions. {\bf C}: Fraction of failed assertions with a counter example. {\bf E}: Fraction of assertions which have syntax errors.}
    \label{tab:result_after_syn_correction}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
         \hline
         \multirow{2}{*}{\bf Designs} & \multicolumn{6}{|c|}{\bf ChatGPT 3.5} & \multicolumn{6}{|c|}{\bf ChatGPT 4.0} & \multicolumn{6}{|c|}{\bf CodeLLaMa2} & \multicolumn{6}{|c|}{\bf LLaMa3-70B} \\
         \cline{2-25}
         \multirow{2}{*}{} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} & \multicolumn{3}{|c|}{\bf 1-shot} & \multicolumn{3}{|c|}{\bf 5-shot} \\
         \cline{2-25}
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E}
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E }
         & {\bf P} & {\bf C} & {\bf E} \\
         \hline
         \input{table/Results_Vaishnavi_06052024_CSV_2}
         %\hline
    \end{tabular}
    }
\end{table}
